Improving Long-Tailed Object Detection with Balanced Group Softmax and Metric Learning

Object detection has been widely explored for class-balanced datasets such as COCO. However, real-world scenarios introduce the challenge of long-tailed distributions, where numerous categories contain only a few instances. This inherent class imbalance biases detection models towards the more frequent classes, degrading performance on rare categories. In this paper, we tackle the problem of long-tailed 2D object detection using the LVISv1 dataset, which consists of 1,203 categories and 164,000 images. We employ a two-stage Faster R-CNN architecture and propose enhancements to the Balanced Group Softmax (BAGS) framework to mitigate class imbalance. Our approach achieves a new state-of-the-art performance with a mean Average Precision (mAP) of 24.5%, surpassing the previous benchmark of 24.0%. Additionally, we hypothesize that tail class features may form smaller, denser clusters within the feature space of head classes, making classification challenging for regression-based classifiers. To address this issue, we explore metric learning to produce feature embeddings that are both well-separated across classes and tightly clustered within each class. For inference, we utilize a k-Nearest Neighbors (k-NN) approach to improve classification performance, particularly for rare classes. Our results demonstrate the effectiveness of these methods in advancing long-tailed object detection.

==> ref.tex <==
% This version of CVPR template is provided by Ming-Ming Cheng.
% Please leave an issue if you found a bug:
% https://github.com/MCG-NKU/CVPR_Template.

% \documentclass[review]{cvpr}
% \documentclass[final]{cvpr}

\usepackage{times}
\usepackage{epsfig}
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{caption} 
\captionsetup[table]{skip=10pt}

% Include other packages here, before hyperref.

% If you comment hyperref and then uncomment it, you should delete
% egpaper.aux before re-running latex.  (Or just hit 'q' on the first latex
% run, let it finish, and you should be clear).
\usepackage[pagebackref=true,breaklinks=true,colorlinks,bookmarks=false]{hyperref}


\def\cvprPaperID{****} % *** Enter the CVPR Paper ID here
\def\confYear{CVPR 2021}
% \setcounter{page}{4321} % For final version only


\begin{document}

%%%%%%%%% TITLE
\title{CSE291J Project Report - Long Tailed Object Detection On LVIS Dataset}

\author{Jessica\\
A53319536\\
{\tt\small jjessica@ucsd.edu}
\and
Satyam Gaba\\
A53305269\\
{\tt\small sgaba@ucsd.edu}
\and
Shrey Garg\\
A53319743\\
{\tt\small sgarg@ucsd.edu}
\and
Tushar Sircar\\
A53267594\\
{\tt\small tsircar@ucsd.edu}
}

\maketitle


%%%%%%%%% ABSTRACT
\begin{abstract}
Object detection problem has been well explored for class balanced datasets such as COCO. However, in the real-world, objects naturally follow a long-tailed distribution - large number of categories and several categories with few instances. Long-tailed object detection is challenging because of the huge class imbalance which leads to the network being biased towards the more frequently occurring classes. In this report, we tackle long-tailed 2D object detection on the LVISv1 dataset (1203 categories, 164K images). We use a two-stage Faster-RCNN network and propose extensions to the SOTA model - Balanced Group Softmax (BAGS) to deal with class imbalance. We are able to improve the overall mAP to 24.50\% as compared to 24.0\% of the SOTA.
We also hypothesise that tail class features might be occurring as smaller clusters within the head class clusters which makes classification hard for a regression-based classifier. We explore metric learning as a potential way to tackle this. This involves learning class features that are well-separated and tight and using KNN inference for classification. The codebase of the project can be found at \href{https://github.com/SatyamGaba/lt_od}{https://github.com/SatyamGaba/lt\_od}

\end{abstract}

%%%%%%%%% BODY TEXT
\section{Introduction}

Object detection is one of the most essential but challenging tasks in Computer Vision. An object detection pipeline involves the following steps:
\begin{itemize}
  \item Finding  bounding boxes
  \item Extracting features for each box
  \item Using these features for classification and bounding box refinement
\end{itemize}

Faster R-CNN\cite{ren2016faster} introduced a Region Proposal Network (RPN) to predict bounding box regions and shared full-image convolutional features with the detection network. This led to two-stage image detectors. On the other hand, single stage detectors such as SSD\cite{liu2016ssd}, YOLO\cite{redmon2016you} take an input image, define a pre-defined set of anchor boxes and predict the class probabilities and refined bounding box coordinates for each anchor box. Generally, these methods are faster than the two-stage methods but are not as accurate. In this work, we primarily focus on two-stage detectors because of their superior accuracy.
A lot of research is underway to improve object detection models but these mostly deal with balanced datasets such as PASCAL VOC\cite{everingham2010pascal} and COCO\cite{lin2014microsoft}. However, in reality, there is a high imbalance in the frequency of image categories and it class distribution tends to follow a long-tailed distribution. The problem of finding efficient models that work well with long tailed datasets is relatively un-explored but important problem to solve.

Recently, the LVIS dataset\cite{gupta2019lvis} was released for work on the long tailed instance segmentation and object detection tasks. It was observed that standard models did not perform well with this dataset as the head classes tend to dominate the tail classes during training. Recent works such as Focal Loss\cite{lin2017focal} and Equalization loss\cite{tan2020equalization} have focused on modifying the cross entropy loss term by assigning higher weights to less confident predictions or by reducing the weight suppression of the tail categories by the head categories. Both these methods perform better than the naive models but accuracy is still not as good as on balanced datasets. Kang et al.\cite{kang2019decoupling} claimed that the class imbalance affects only the classification and not the feature representation learning part of the network. They decouple representation learning and classifier training and show that it's an effective strategy for the long tailed detection task. After learning representations with the naive model, the feature extraction layers are frozen and the classifier head is fine-tuned while normalizing the weights between head and tail classes. Another approach to long-tailed detection is to facilitate the direct transfer of knowledge from the head classes to the tail classes. This is proposed in \cite{learning2segment}. The categories are divided into groups based on instance frequency and the model is trained in phases - group by group. At subsequent stages, the samples from previously seen categories are replayed in a class-balanced way so that the network doesn't forget them. Additionally, the classifier weights for tail classes are learn as a linear combination of the classifier weights of head classes.
While this approach gets decent results, it is reliant on tail categories being visual similar to head categories which might not always be true.
Recently, \cite{li2020overcoming} introduced a novel classification loss (Balanced Group Softmax) in which the image categories were divided into bins based on image frequencies and softmax loss was computed for each bin separately. Since, images in a bin only compete with other categories (having similar frequencies) in the bin, this mitigates the long tailed problem. This method is the state of the art for long tailed object detection. 

However, we felt that there was scope for improvement in the balanced group softmax model and hence performed further ablation studies. Detailed studies and logic for the choice of bins was not shown. Hence, we have experimented with different number of bins in the BAGS model. We have also tried a novel clustering method to categorize images into bins. We realized that even though the bins were reducing the long tailed detection problem, it still existed within a bin. Hence, we implement multiple variants of 'weighted BAGS' which uses popular loss weighing methods inside each bin. Using this weighing, we are able to improve the rare and common classes AP by around 1.25\%. 

We realize that we need to think of better methods that focus on solving and not reducing the long tailed distribution problem. We explore metric learning for object detection. We add additional Center Loss\cite{wen2016discriminative} and Cos Loss\cite{wang2018cosface} to our training methods and perform experiments to determine their effectiveness. We also introduce a noval 'Euclidean cross entropy' loss that tries to minimize the intra class distance between image features.
We use K nearest neighbours as well as Cross entropy for inference and explain our results and observations.

% - object detection pipelines
% - two-stage , one-stage models
% - SSD, Faster-RCNN
% - losses
% - long-tailed object detection ( summary of papers we read)
% - describe problem in learning tail classes
% - mention two types of exp :
%     - bags experiments
%     - metric learning



\section{Development Process}
\begin{figure*}[h]
\includegraphics[width=\textwidth]{figures/tls.PNG}
\caption{Development Process - Timeline}
    % \label{fig:my_label}
\centering
\end{figure*}

\subsection{Weeks 1-2}
Weeks 1-2 involved going through understanding the long-tailed object detection problem and getting to know team. We spent time on reading and analyzing existing literature to understand existing object detection pipelines and review state of the art methods in long-tailed object detection. We studied existing one-stage and two-stage object detection networks such as Faster-RCNN, YOLO and Single Shot Detector (SSD). We decided to move-forward with two-stage detectors as they tend to perform better.

After getting a good understanding about the object detection pipeline, we read up about existing methods to deal with class imbalance such as under/over-sampling, re-weighting, repeat factor sampling and alternate loss functions. 

We then moved on to review previous solutions to the LVIS long-tailed detection challenge. We reviewed Balanced Group Softmax (BAGS), Learning To Segment, Decoupling based methods, Focal Loss and Equalization Loss.
Based on our review, we decided to build up on the state of the art Balanced Group Softmax model.

\subsection{Weeks 3-5}
Following this, in weeks 3-5, we evaluated existing object detection libraries MMDetection and Detectron2. Since most of the long-tailed detection code-bases were based on MMDetection, we decided to use MMDetection object detection library for our experiments. We got familiar with the library by running small experiments on it. More specifically, we trained a Faster-RCNN model from scratch to learn a single COCO dataset category and also fine-tuned an existing Faster-RCNN model trained on the COCO dataset to learn a new LVIS dataset category. We also visualized the features produced by the network.
Next, we got familiar with using the Nautilus cluster, debugged several GPU and memory related issues, and used the MMDetection library to train the Faster-RCNN baseline model and decoupling (tau-normalization) methods on LVIS. 
The code-base for the Balanced Group Softmax code-base is designed for LVIS-V0.5 and an older version of MMDetection. Our next step was to port this model to the newer version of MMDetection. This involved understanding how the method was implemented and making relevant changes to the newer MMDetection version. We then trained the model with BAGS to get our benchmark SOTA results on LVIS-V1. 

\subsection{Weeks 6-8}
In weeks 6-8, we experimented with several extensions to the BAGS model. We observed that BAGS divides categories into groups and applies per-group softmax to reduce inter-group imbalance but doesn't address the intra-group imbalance that remains. To tackle this, we extend BAGS with class-weights, focal loss and try alternate bin configurations by changing the number of bins and etc. We were able to achieve better results than the BAGS method. We ran multiple models with different parameters and produced results.

\subsection{Weeks 9-10}
In weeks 9-10, we explored metric learning for object detection. We read up about Center Loss and Large-Margin Cosine Loss and used these to generate well-separated and tight feature clusters. We implemented KNN inference for classification based on this.
Further, we visualized features and tried to analyze the limitations of metric learning empirically. We also propose cross-entropy euclidean loss for implicitly optimizing the model for nearest neighbor classification.


% - initial setup and survey
%     - paper reviews, selecting to move forward with BAGS
%     - short description about mmdetection library. 
%     - setting up mmdetection
%     - Migration on BAGS to mmdet v2
% - reproduce baselines
%     - Identifying baseline - faster rcnn
%     - decoupling classifier
% - ablation studies
%     - random BAGS ablation to see effectiveness of groups
%     - change number and structure of bins

% - Dealing with imbalance within the bins
%  - BAGS with class weights
%  - Hybrid (for frequent classes)
%  - Focal loss

% - Metric learning
%     - visualizing features gave idea of metric learning
%     - idea behind using metric learning
%     - center loss
%     - cos loss
%     - euclidean cross entropy loss
%     - feature  visualizations

\section{Method}

\subsection{Baseline Model - Faster-RCNN}

Faster RCNN network architecture can divided into three networks, each responsible for a different task. Backbone architecture for extracting feature maps out of the input image, Region Proposal Network (RPN) for generating region proposals and ROI head network, responsible for bounding boxes regression and classification of objects.\par
Backbone is typical a convolutional neural network such as VGG16, ResNet50, that extracts feature maps from the input image. ResNet backbone are chosen over VGG because they can handle vanishing gradients problem of a deeper network. Backbone generates anchors, uniformly distributed over the entire image. First, the network generates a grid of anchor points on the image and then, generate anchor boxes for each anchor point. At each anchor point there are multiple anchor boxes of multiple scale/size and height to width ratio as shown in Figure  \ref{fig:anchors}.\par
\begin{figure}[h]
    \centering
    \includegraphics[width=0.3\textwidth]{figures/anchors.png}
    \caption{Anchor boxes of three different sizes and height to width ratio at an anchor point}
    \label{fig:anchors}
\end{figure}

The features from the backbone model and the anchor boxes are fed into RPN to generate proposals for objects. The output of the RPN is a bunch of boxes/proposals that will be examined by a classifier and regressor in ROI head to eventually check the occurrence of objects. To be more precise, RPN predicts the possibility of an anchor being background or foreground, and refine the anchor.\par
The RPN produces an arbitrary constant number of proposals for every image. ROI head takes top proposals with highest probability of occurrence of object. ROI head has a classifier and a bounding box head for image category classification and final bounding box regression respectively. In classifier head, the feature are converted in linear layers of the size of number of categories. Cross Entropy loss is applied at the end of classifier head for training. Whereas in bounding box head the corresponding anchors are regressed to fit to the ground truth bounding box. We use L1-smooth loss for bounding box regression head.\par
Faster-RCNN can be trained in two different ways: alternatively train the RPN, and the final classifier and regressor; train them at the same time jointly. We use the later because it is faster with similar accuracy. The gradients back propagate to the CNNs in both ways.\par

% - description of baseline method
%     - backbone
%     - rpn
%     - bbox and classifier heads

\subsection{Decoupling Classifier}

It has been found that the bias in classifier towards head classes is developed due to imbalances in weights norms of classifier. The classifier weight norm corresponding to head classes are higher than tail classes\cite{kang2019decoupling}. Decoupling classifier approaches claim that the imbalance affects classification but not the feature representation learning. It trains the feature extraction network using standard cross-entropy loss, freezes the feature extraction layers and then re-trains the only the classifier head to mitigate the difference in classifier's weight norms for head and tail classes. This is done by re-training the classifier head on a re-sampled balanced data distribution. 
\cite{kang2019decoupling} considers the following approaches to sample a balanced dataset for retraining the classifier: (1) Instance-balanced sampling; (2) Class-balanced sampling; (3) Square-root sampling; (4) Progressively-balanced sampling.\\
Rebalancing classifier's weight norms methods such as (1) Classifier re-training (cRT); (2) Nearest Class Mean classifier (NCM); (3) 
$\tau$-normalized classifier ($\tau$-normalization); and (4) Learnable weight scaling (LWS) exhibit better results for the tail classes. We chose to experiment with Tau-normalization because of its superior performance and no training over-head \cite{kang2019decoupling}.
\subsubsection*{Tau normalization}
Tau normalization does not require retraining the classifier. It uses the joint-trained model and reweighs at classifier weights during inference. This method normalizes the weight across all categories by dividing weight by their respective norms. There is a temperature value ($\tau$) between 0 to 1, that controls the amount of normalization. The updated classifier weights will be:
\begin{equation*}
    \hat{w} = w/|w|^{\tau}
\end{equation*}
Higher the value of $\tau$, more uniform distribution weights as shown in Figure \ref{fig:tau_norms}.\\
With Tau-normalization there is no overhead during training or inference time.
\begin{figure}
    \centering
    \includegraphics{figures/tau_norms.png}
    \caption{Weight norms for each category with different values of $\tau$. Categories are sorted according to instance count}
    \label{fig:tau_norms}
\end{figure}
\subsection{Benchmark Model - Balanced Group Softmax}   
Standard softmax loss, used by the baseline Faster-RCNN model, is not suitable for long-tailed detection. This is because learning for the tail classes are dominated by negative gradients being generated by the head classes. This leads to highly skewed classifier weight norms (correlated to the instance count) and consequently poor performance (close to 0 mAP) for the rare categories.\par
The Balanced Group Softmax (BAGS)\cite{li2020overcoming} loss divides categories into groups based on frequency and does group-wise training. Since categories with similar frequencies are in the same group, it eliminates the domination caused by the negative head class gradients.\par
More formally, $C$ categories are divided into $N$ groups. Category $j$ belongs to group $G_{n}$ if the number of instances of category $j$ is in the range $[s_{n}^{l}, s_{n+1}^{l})$ where $s_{n}^{l}$ is the lower bound on the instance frequencies for $G_{n}$. The best results on LVIS as reported in \cite{li2020overcoming} are with $N = 4$ and $s_{1}^{l} = 0, s_{2}^{l} = 10, s_{3}^{l} = 100, s_{4}^{l} = 1000$.\par
The background category is assigned to $G_{0}$.
Also, each group has an 'Others' category that refers to all categories not included in the group.
While training, for a proposal with ground truth label $c$, only two groups will be activated - $G_{0}$ and $G_{n}$ where $c \in G_{n}$.
Within these groups, softmax cross-entropy loss is computed. 
For most groups, the 
Additionally, for each batch, the number of 'Others' samples used is limited to avoid creating another imbalance problem.

The output of the network is $z \in {\rm I\!R}^{(C+1)+(N+1)}$. The probability of class $j$ is calculated as:
$$p_{j} = \frac{e^{z_{j}}}{\sum_{i \in G_{n}} e^{z_{i}}}$$ where, n is such that $j \in G_{n}$. In groups where category $c$ is not included, the 'Others' class is treated as the ground truth class.
Then the final loss is:
$$L_{k} = -\sum_{n=0}^{N}\sum_{i \in G_{n}}y_{i}^{n} log (p_{i}^{n})$$ where $y^{n}$ and $p^{n}$ represent the label and probability in $G_{n}$.

\subsection{Extensions To BAGS Loss}

The process of applying softmax to each bin independently (as done in BAGS) tackles the problem of inter-group class imbalance by not letting frequent classes dominate the infrequent ones during training. But even within a bin, class imbalance exists as the data is large and instance frequency within a bin varies greatly. This is depicted in Figure \ref{fig:intra-bin-imbalance}.

\begin{figure}[h!]
  \includegraphics[width=\columnwidth]{figures/intra-bin-imbalance.pdf}
  \caption{Class distribution imbalance within groups/bins generated by the Balanced Group Softmax method. }
  \label{fig:intra-bin-imbalance}
\end{figure}

To handle the imbalance within each bin, we experimented with several methods which are described in the following sub-sections.


\subsubsection{Altering Number Of Bins For BAGS}

The splits in the optimally performing BAGS model has 4 bins based on 10, 100, 1000 and 10000 instance counts\cite{li2020overcoming}. A simple way to reduce intra-group imbalance is to increase the number of bins. 
The paper experiments with 8 bins but it creates the problem of having too few samples in some bins which leads to poor performance.

Instead, we approached the task of increasing the number of bins by splitting the bin with most number of samples i.e. the bin with 100-1000 instance counts. It was split into two bins corresponding to categories with 100-500 and 500-1000 instance counts.
We re-generated mappings of labels to their corresponding bin labels and trained the classification head with the newly defined bins.

% BAGS benefits from the group-wise training of categories because it essentially separates the training if tail classes from the head. To improve the classification performance even further, we experimented with different distributions of categories within bins and a different number of bins. The aim behind the experiment being to leverage the separation of training to its maximum.


\subsubsection{Clustered BAGS}

In BAGS\cite{li2020overcoming}, no ablation study was done by varying the frequency ranges inside each bin. Decision boundaries like 10, 100, 1000 were trivially chosen. We observed that the tail categories in each bin did not have high AP's and this method tries to reduce the number of tail categories per bin. With clustered BAGS, we clustered the image categories based on instance frequencies. Moreover, we ensured that clusters chosen had less number of image categories for the tail frequencies. This would ensure that a lot of categories are not adversely affected because of the long tail distribution inside each bin. We used the following thresholds for our bins: 0-22, 23-90, 91- 1000, 1001-18050 and 18050++.


\subsubsection{BAGS With Class-Weights}

In this approach, to handle the imbalance within each bin, we decided to employ a classic approach - class weighting. Each class is weighted by the inverse of its instance frequency, effectively lowering the weight given to frequent categories within a bin. This ensures that the contribution of frequent categories does not dominate the loss. More formally, we calculate the weight assigned to each class as follows.
For each class, we initialize the weight to the inverse of the instance count. Let $w_{init}(i)$ denote the weight of the i-th class.
Then, within each bin, we normalize the weights so that they sum up to 1.
$$w_{normalized}(i) = \frac{w_{init}(i)}{\sum_{j \in G_{n}}w_{init}(j)}$$.
When no weights are used, effectively we are giving a weight of 1 to each category and the weights of categories in a group sum up to the number of categories in that group. To ensure that the overall weight to the loss term hasn't decreased, we re-scale these weights by the number of categories in the particular group.
$$w_{final} = w_{normalized}(i) * |G_{n}|, i \in G_{n}$$.
These final weights are used while training.

\subsubsection{BAGS With Focal Loss}

In this approach, we use Focal Loss\cite{lin2017focal} for classification within bins. This loss dynamically puts more emphasis on harder mis-classifier examples and less emphasis to well classified or easy examples. 
Thus, it inherently weighs the less frequent categories more as they are harder to classify. Additionally, even for head classes, some objects might be harder to classify than others and this loss gives more importance to those samples.


More formally, focal loss can be defined for binary classification as: 
\[ FL(p_{t}) = -(1-p_t)^\gamma log(p_t)\]
where \(\gamma\) is a tunable focusing parameter and \(p_t\) is the probability of the sample belonging to the category so that \(CE(p_t) = -log(p_t)\) and \(p_t\) is \(p\) or \(1-p\) according to the class label\cite{lin2017focal}.

When an example is mis-classified and \(p_t\) is small, the
modulating factor is near 1 (more importance). As
$p_{t}$ → 1, the factor goes to 0 and the loss for well-classified
examples is down-weighted. 


% - metric learning
%     - center loss + CE ( different weights)
%         - Inference with CE
%         - Inference with KNN
%     - Cos loss (w and w/o CE)
%         - Inference with CE
%         - Inference with KNN
%     - Euclidean CE loss.
%         - Inference
        
\subsection{Metric Learning}

Object detection involves classification and bounding box regression. However, it might be that the features of tail classes appear as smaller clusters close to or within the relatively large clusters of the head class as shown in Figure \ref{fig:metric-learning-hypothesis}.
The last layer of the classification head has to learn a linear decision boundary based on these features which might not be sufficient for classification.
In this case, nearest neighbor classification would be more appropriate. However, for nearest neighbor classification to be effective, the features of different categories should be well-separated. With this in mind, we explore Center Loss\cite{wen2016discriminative} and Large Margin Cosine Loss\cite{wang2018cosface} as described in upcoming sub-sections.

\begin{figure}[h!]
  \includegraphics[width=\columnwidth]{figures/metric-learning-hypothesis.png}
  \caption{Tail class feature cluster occurring within or at the boundary of head class feature cluster. The blue dots represent the head class and others represent tail classes.}
  \label{fig:metric-learning-hypothesis}
\end{figure}

\subsubsection{Center Loss}
Softmax cross-entropy loss tries to ensure that the features of different classes are well-separated in space.
However, it doesn't ensure that the feature clusters are tight.
In Center Loss, we keep track of the feature center of each class and try to minimize the distance of features from their corresponding class centers.
More formally, center loss is defined as follows:
$$L_{Center} = \frac{1}{2}\sum_{i=1}^{m}||x_{i} - c_{y_{i}}||_{2}^{2}$$
where $c_{y_{i}}$ denotes the center of the $y_{i}$-th class's deep features.
The class centers are updated in each iteration based on the mini-batch instead of computing it over the entire dataset every time\cite{wen2016discriminative}.

The model is trained with a combination of softmax cross-entropy and center loss as follows.

$$L = L_{softmax} + \lambda L_{Center}$$.
We perform inference in two ways. 
\begin{itemize}
    \item Method 1 is to take arg-max over the soft-max scores (ignoring the centers) during inference.
    \item Method 2 is KNN inference. For this, we compute the centers by keeping track of the running feature means for each  center. For a given bounding box, the score assigned to a class is equal to the negative of the distance from the corresponding center. We then apply softmax over it to compute the probability for each class.
\end{itemize}

\subsubsection{Large Margin Cosine Loss}
For tasks like facial recognition, new losses such as center loss outperformed conventional softmax losses because of there ability to better discriminate the features. These losses are based on the idea: maximizing inter-class variance and minimizing intra-class variance. Large Margin Cosine Loss (LMCL)\cite{wang2018cosface} reformulates the softmax loss as a cosine loss by L2 normalizing both features and weight vectors to remove radial variations, after which a cosine margin term is introduced to further maximize the decision margin in the angular space.\\
The LMCL is defined as:
\begin{equation*}
    L_{l m c}=\frac{1}{N} \sum_{i}-\log \frac{e^{s\left(\cos \left(\theta_{y_{i}, i}\right)-m\right)}}{e^{s\left(\cos \left(\theta_{y_{i}, i}\right)-m\right)}+\sum_{j \neq y_{i}} e^{s \cos \left(\theta_{j, i}\right)}}
\end{equation*}

LMCL achieves minimum intra-class variance and maximum inter-class variance by virtue of normalization and cosine decision margin maximization as shown in Figure \ref{fig:cos_loss_vis}.\par


\begin{figure}[h]
    \centering
    \includegraphics[width = 0.5\textwidth]{figures/cos_loss_vis.png}
    \caption{ A toy experiment of different loss functions on 8 identities with 2D features. The first row maps the 2D features onto the Euclidean space, while the second row projects the 2D features onto the angular space. The gap becomes evident as the margin term m increases.\cite{wang2018cosface}}
    \label{fig:cos_loss_vis}
\end{figure}


\subsubsection{Euclidean Cross Entropy Loss}
\[ ECE = - \sum_{i=1}^{m} \log{\left( \frac{ e^{\frac{-||x_i - w_{y_i}||^2}{t}} }{ \sum_{j=1}^{m} e^{\frac{-||x_i - w_{y_j}||^2}{t}} } \right)}
\]


The idea behind this loss is to consider the numerator in the softmax term of Cross Entropy Loss $(w_ix_i)$ as the un-normalized cosine distance between weight and feature vectors. Instead of having this cosine distance, this loss uses a Euclidean distance from the learned parameters $w_{y_i}$ 

\section{Experiments}

\subsection{Reproduced Baseline and SOTA}    
We trained Faster-RCNN model on LVIS dataset for 12 epochs. We used 4 GPUs with a batch size of 2 images per GPU. Learning rate was set to 0.025 as suggested by the MMDetection library.
Overall mAP was calculated along with mAP for the rare, common and frequent categories. 
We also trained the balanced group softmax model (SOTA) on the LVIS-V1 dataset. The results for these are shown in Table \ref{table:reproduce}. It can be observed that the BAGS model boosts the overall mAP and almost doubles the mAP for rare categories.
While the original BAGS paper experimented on LVIS -V0.5, the results are pretty close in performance.
 
\begin{table}[h!]
\centering
 \begin{tabular}{|c | c | c | c | c|} 
 \hline
  & Overall & Rare & Common & Frequent \\
 \hline
 Baseline & 21.1 & 8.1 & 19.6 & 28.6 \\
 \hline
 BAGS & 24.0 &  15.6 & 22.8 & 29.2 \\
 \hline
\end{tabular}

\caption{mAP values obtained on LVIS-V1 validation set with baseline Faster-RCNN and BAGS model.}
\label{table:reproduce}
\end{table}



\begin{table}[]
\centering
\begin{tabular}{|l|l|l|}
\hline
$\tau$       & mAP                           & APr                          \\ \hline
0 (baseline) & \cellcolor[HTML]{9E9E9E}21.1 & 0.9                        \\ \hline
0.05         & 20.0                           & 0.9                        \\ \hline
0.1          & 19.8                         & 1.1                        \\ \hline
1            & 12.8                         & \cellcolor[HTML]{9E9E9E}4.0 \\ \hline
\end{tabular}
\caption{Tau normalization results on validation data. AP for rare categories (APr) increases when $\tau$ value increases. However, mean AP value (mAP) decreases with increase in $\tau$ value.}
\label{table:tau_norm}
\end{table}

\subsection{Decoupling - Tau Normalization}
We experimented with different values of $\tau$ to observe it's effectiveness on tail classes. We implemented $\tau$-normalization during inference on the baseline model.
Table \ref{table:tau_norm} shows the mean AP (mAP) and AP on rare categories (APr). APr value improves with increasing $\tau$ value, however mAP value decreases. This is expected as we trade off performance on head categories for tail categories and since, head categories are in abundant therefore they deplete mAP more than tail categories improve it.

\subsection{Ablation Studies: Random BAGS}

To test the effectiveness of sorting the categories by instance frequency before dividing them into bins, we performed an ablation study where the sizes and number of bins were kept same but the distribution of categories into bins was made random. 

Table \ref{table:rags} shows the comparison of results on this randomly divided model with the original BAGS results. The AP for rare classes has dropped drastically, and that follows from common sense because tail classes would be suppressed whatever bin they may be assigned. 

Frequent classes AP has increased which is also intuitive as they will be able to dominate more classes if they are spread out evenly rather than competing among themselves.
 
\begin{table}[]
\centering
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{}     & Overall & Rare & Common & Frequent                     \\ \hline
BAGS & 24.0    & 15.6 & 22.8   & \cellcolor[HTML]{FFFFFF}29.2 \\ \hline
RAGS          & 19.8    & 2.6  & 17.8   & 29.6                         \\ \hline
\end{tabular}
\caption{Comparison of BAGS with Random BAGS (RAGS) for which bin distribution is random and not based on instance frequency.}
\label{table:rags}
\end{table}

\subsection{Extensions To BAGS}
Table \ref{table:bags-mod} indicates the overall mAP and mAP for the rare , frequent and common categories obtained via the BAGS extensions described in Section 3.5. 
We observe that each method specializes in for a different set of categories. For example, BAGS with class-weights improves mAP for rare and common categories but leads to a deterioration in mAP for frequent categories. 
Based on this observation, we adopt a hybrid approach where we use softmax with class-weights for rare and common categories and apply standard softmax for the frequent categories. This further improves overall mAP to 24.5\%.



\begin{table}[]
\centering
\begin{tabular}{|l|l|l|l|l|}
\hline
Modification & Overall                      & Rare                         & Common                       & Frequent                     \\ \hline
Original          & 24.0                         & 15.6                         & 22.8                         & \cellcolor[HTML]{9E9E9E}29.2 \\ \hline
5-Bins            & 24.2                         & 15.6                         & 23.1                         & 29.1                         \\ \hline
Clustered            & 24.0                         & 15                         & 23                         & 29.1                         \\ \hline
Focal loss        & 24.0                         & \cellcolor[HTML]{9E9E9E}16.4 & 23.2                         & 28.2                         \\ \hline
Class weighted & \cellcolor[HTML]{9E9E9E}24.3 & 16.1                         & \cellcolor[HTML]{9E9E9E}23.6 & 28.7                         \\ \hline
\rowcolor[HTML]{EFEFEF}
Hybrid            & \cellcolor[HTML]{9E9E9E}24.5 & 16.6                         & 23.1                         & 29.4                         \\ \hline
\end{tabular}
\caption{mAP values obtained on LVIS-V1 validation set with proposed extensions to the BAGS model - 5 bin configuration, clustered BAGS, focal loss and class-weights. The highlighted cells indicate the best results obtained (excluding the hybrid approach) for the category set corresponding to that column.}
\label{table:bags-mod}
\end{table}




\begin{figure}
    \centering
    \includegraphics{figures/bags_weights.png}
    \caption{Classifier weights visualization}
    \label{fig:my_label}
\end{figure}

\subsection{Metric Learning}

\subsubsection{Center Loss}

We trained Faster-RCNN model with Center Loss for 12 epochs. The feature dimension used for center calculation and KNN inference was 1024. We first trained the model on a subset of 30 categories randomly selected from the LVIS-V1 dataset. We tried multiple values for the weight assigned to center loss ($\lambda$) - 0.1 and 0.01.
As described in the previous section, we did both softmax based inference and KNN inference. The results are shown in the first four rows of Table \ref{table:knn}.

On a 30-category subset , we observe that KNN improves mAP for rare and common classes as compared to softmax inference. However, overall mAP was still higher for standard softmax inference.

We re-train the model on the entire dataset as well with $\lambda = 0.01$. The results are indicated in the last row of Table \ref{table:knn}. We observe similar results as that on the 30-category subset.
We tried to analyze the reason for this by visualizing the class features. We extract features and plot them in 2D using tSNE transformations.


Feature visualization (shown in Fig.\ref{fig:tsne}) suggests that  tail classes do not cluster as well as expected. They are more scattered and have a high variance. 
This is intuitive as certain tail classes, such as cucumbers Fig.\ref{fig:cucumber}, appear in several different shapes, sizes and textures across multiple instances.
Moreover, the dataset has 1203 classes, and naturally some categories will have similarities which further makes it difficult to have completely separated clusters. Nearest neighbor classification is not as powerful if the feature clusters are not completed isolated which explains the poor mAP values. 


\begin{table}[]
\centering
\begin{tabular}{|l|l|l|l|l|l|}
\hline
Method & $\lambda$ & Overall & Rare                        & Common & Frequent \\ \hline
Softmax          & 0.01               & 14.7    & 0.0                         & 13.4   & 23.6     \\ \hline
Softmax          & 0.1                & 5.8     & 0.0                         & 1.7    & 13.5     \\ \hline
KNN              & 0.01               & 9.8     & \cellcolor[HTML]{B7B7B7}1.5 & 5.6    & 19.0     \\ \hline
KNN              & 0.1                & 2.4     & 0.0                         & 0.0    & 6.6      \\ \hline
\rowcolor[HTML]{EFEFEF} 
KNN  & 0.01         & 5.0     & 0.0                         & 0.01   & 12.6     \\ 
\rowcolor[HTML]{EFEFEF} 
(all data) &  & & & & \\ \hline
\end{tabular}
\caption{Comparison of inference of models trained with Center Loss with specified weight $\lambda$ and Cross Entropy Loss using KNN and Softmax methods. The first four rows correspond to models trained on a 30 category subset of data. The last row corresponds to the model trained on the entire dataset with $\lambda = 0.01$.}
\label{table:knn}
\end{table}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.3\textwidth]{figures/tsne.png}
    \caption{tSNE visualization of category features for 9 categories. It can be observed that the tail class features are scattered and don't appear in a tight cluster.}
    \label{fig:tsne}
\end{figure}


\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/cucumber.png}
    \caption{Variations in color, texture and shape for 'cucumber' class instances.}
    \label{fig:cucumber}
\end{figure}


\section{Future work}
Metric Learning is a powerful tool that can be helpful for the long tail object detection task, but we will need to understand it better. There is a need to theoretically understand the high dimensional space of the features. Nearest neighbor inference might not be useful since the distribution might be multi-modal and we might need to account for multiple centers. 
Another idea that we wish to work on is representing the tail class features as a linear/nonlinear combination of the head class features. This will allow us to use the head class data to enrich results for the tail classes.
Another strategy is to do more aggressive data augmentation. Since segmentation masks of objects are known, they can be replicated on to different backgrounds and poses to increase the instance frequency.
We also plan to leverage segmentation masks present in the LVIS dataset to enrich our training set. This should help us get better bounding box and classification accuracy.

% - Evaluate metric learning theoretically and conclude
% - Other Ideas from few-shot learning 


\section{Appendix}
\subsection{Individual Contribution}

\subsubsection{Jessica}
During the first few weeks, Jessica focused on classifier modifcations for the literature review. To better understand the mmdetection codebase, she and Satyam worked on overfitting a model on a single image. 

Following that, she worked on making changes in codebase to use pretrained models trained on older mmdet versions migration. She contributed to chaging the mmdetection inference code to obtain classwise AP results and per image AP results and at a later stage, also improving its space complexity. 

She also worked on reproducing tau normalization results and on the migration of bags model to newer versions of mmdet and lvis which involved making changes to the bin creation code and the classifier head code. 

For BAGS modifications she worked on experimenting with different number of bins and comparing and visualizing classwise performance among the different modifications. 

When the team switched tracks towards metric learning, she collaborated with Satyam on implementing and training the bags model using large margin cosine loss to separate the features. The following week they collaborated again on implementing the new Euclidean Cross Entropy Loss. She also contributed to the feature visualization script.

\subsubsection{Satyam}
During initial weeks, Satyam did Literature survey and reviewed the basics of object detection. He reviewed repositories for various papers to better understand their approaches. Then a week was spend in understanding the mmdetection toolbox. He was partnered with Jessica and worked on overfitting a model on a single image and gained insights. Backbone Feature visualization was also done for better understanding. After that, he contributed in creating a baseline model for object detection on lvis dataset using faster-rcnn (masked-rcnn given in mmdetection).\par
Satyam and Jessica worked on decoupling the classifier approach. They implemented tau normalization for various values of tau. He contributed in migrating code from balanced group softmax paper's repository to newer version of mmdetection and lvis v1 dataset. He did ablation studies and contributed in importing focal loss to BAGS\par
Lastly, Satyam worked with Jessica on metric learning, especially large margine cosine loss, euclidean cross entropy loss. Other contributions of Satyam were APIs for category-wise AP, class-wise AP, feature visualization. He worked on solving memory leakage problem in LVIS API and optimized it. He also contributed in weekly presentations and group discussions

\subsubsection{Shrey}
Performed literature Review of recent long-tailed object detection papers. Spent time understanding mmdetection and its various modules. Performed baseline experiements like fine-tuning COCO model for LVIS categories to get a good understanding of mmdetection. 

Worked on BAGS training using the old and new mmdetection versions. Helped port selective training of BAGS classifier to the new mmdetection version. Spent a bit over a week debugging multi-gpu training issues and issues arising due to memory on Nautilus. After environment was set up, trained BAGS while freezing different parts of baseline and analyzed results. Visualized and understood bin formation in BAGS. Realized that a lot of tail frequencies in each bin have a lot of categories associated with them. Proposed, implemented, trained and performed inference on Clustered BAGS to solve the above issue.

Worked on center loss+BAGS model inference.  Implemented the K-Nearest neighbour inference method for the clusters formed. Performed inference using the Cross Entropy loss and compared results with the ones obtained during KNN. Visualized image features with and without center loss and tried to understand if adding the loss made a significant difference to the features. Performed experiments to check why KNN was not working well. There included finding average distances between cluster centers and distance between image features and clusters for a subset of categories.


\subsubsection{Tushar}
Did literature review of existing long-tailed detection papers and read up on submissions to LVIS challenge. Understood object detection pielines, MMDetection library (fine-tuned pre-trained COCO model to learn an LVIS category) and ported BAGS inference code to the newer version of MMDetection. Spent some time trying to debug why multi-GPU training wasn't working.

Made relevant configuration changes and trained Baseline (Faster-RCNN) model and Balanced Group Softmax models on Datahub and Nautilus.  Generated bins based on a random distribution and trained random BAGS model (RAGS) for ablation study. Analyzed category-wise AP values to identify worst and best performing categories within each bin. Analyzed errors of benchmark models by visualizing bounding boxes of categories whose instance count was high yet AP was low (cucumbers, bell peppers etc.). 

Visualized class distribution within bins, realized that there was an imbalance and proposed the idea of extending BAGS to deal with intra-class imbalance. 
Implemented BAGS with class-weights - this involved generating a per-class weight configuration file that assigned classes weights based on the instance frequency and category count within each group and using the loaded weights to modify the loss function in BAGS. This gave better overall mAP than the SOTA.
Noticed that different methods specialize for different categories and implemented the hybrid of class-weights and standard softmax to further improve the overall mAP to 24.5\%.

Implemented center loss and trained models with center loss on a 30-category subset as well as the entire dataset with multiple values of the hyper-parameter $\lambda$. Additionally, implemented KNN classification for inference with Center Loss. This involved keeping track of the class centers on the fly and assigning scores based on distance followed by softmax for classification.
Visualized features learnt by center loss to analyze why KNN wasn't performing as well. Identified the reason to be high variance in tail classes.



\subsection{Suggestions to Improve the Course}

Since, the course was offered first time, there were issues getting multiple GPU initially. Given our requirements, we needed upwards of 50 GB memory for each training session. It was really tough to get such high memory on Nautilus. Moreover, during the first few weeks, Nautilus was a bit unstable and this limited our progress.



% {\small
% \bibliographystyle{ieee_fullname}
% \bibliography{egbib}
% }




\end{document}

